Stochastic Image-to-Video Synthesis using cINNs

Video understanding calls for a model to learn the characteristic interplay between static scene content and its dynamics: Given an image, the model must be able to predict a future progression of the portrayed scene and, conversely, a video should be explained in terms of its static image content and all the remaining characteristics not present in the initial frame. This naturally suggests a bijective mapping between the video domain and the static content as well as residual information. In contrast to common stochastic image-to-video synthesis, such a model does not merely generate arbitrary videos progressing the initial image. Given this image, it rather provides a one-to-one mapping between the residual vectors and the video with stochastic outcomes when sampling. The approach is naturally implemented using a conditional invertible neural network (cINN) that can explain videos by independently modelling static and other video characteristics, thus laying the basis for controlled video synthesis. Experiments on four diverse video datasets demonstrate the effectiveness of our approach in terms of both the quality and diversity of the synthesized results. Our project page is available at https://bit.ly/3t66bnU.

==> chapters/method_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% Preamble for method section %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Modelling this dual relationship between the image and video domain essentially calls for a bijective transformation. Since the content information captured in an image only represents a subset of the video domain, learning such an invertible mapping requires a dedicated residual representation modelling the lacking dynamics information. Once being established, given an initial image and an dynamics representative, we can synthesize the corresponding future video sequence. Further, having observed a video sequence, we can explain its scene dynamics by means of the residual representation given its initial image. 

We want to understand the image-to-video synthesis problem by learning a bijective transformation between images and their potential future progression depicted in video sequences. Following, we present how to efficiently learn such a mapping by means of deep neural networks.

\subsection{Image-to-Video Synthesis}
Bijective transformations are invertible, unique one-to-one mappings between two structured domains. However, given an initial image $x_0 \in \mathbb{R}^{d_x}$ there are many possible ways how the depicted scene could be progressing, thus being mapped to a counterpart $X = [ x_1,\dots,x_T ]$ in the video domain. Consequently, to fulfill the bijection property, we have to introduce a dedicated \emph{dynamics representation} $\nu \in \mathbb{R}^{d_\nu}$ compensating for this ambiguity. Moreover, due to the high dimensionality of video sequences entailing lots of redundant information, we assume videos to be fully described by a learned, compact representation $z \in \mathbb{R}^{d_z} $, i.e. $z$ allows to faithfully reconstruct $X$. Based on this,  $\nu$ and $x_0$ \emph{together} define the unique mapping $\mathcal{T}: \mathbb{R}^{d_x} \times \mathbb{R}^{d_\nu} \mapsto \mathbb{R}^{d_z}$ with
%
\begin{equation}
z = \mathcal{T}(x_0; \nu) \;.
\label{eq:imagetovideo2}
\end{equation}
%
To model the stochastic nature of the synthesis process, we assume realizations of $\nu$ to be drawn from a probabilistic model
%
\begin{equation}
\nu \sim p(\nu|x_0) \; .
\end{equation}
%
We can now translate the image-to-video synthesis problem to learning the distribution of $\nu$ such that the invertible mapping $\mathcal{T}$ can be established.
\paragraph{Inferring An Explicit Dynamic Representation}
Recall that $\nu$ should capture all the residual information in the full video representation $z$ which \emph{cannot} be described by the starting frame $x_0$. This implies that $\nu$ can be determined as the inverse of Eq.~\eqref{eq:imagetovideo2}
%
\begin{equation}
\nu = \mathcal{T}^{-1}(z;x_0), 
\label{eq:backward}
\end{equation}
%



We want to learn a mapping $\mathcal{T}$ which, given an input image $x_0$, predicts likely future frames $x_1, \dots, x_T$, i.e.\
\begin{equation}
\mathcal{T}: x_0 \mapsto \{x_1, \dots, x_T\}
\label{eq:imagetovideo}
\end{equation}
Given that visual data is high dimensional and complex we seek for a redundancy-free, compact video representation $z_{\nu}$, from which a video $x_0, \dots, x_T$ can be faithfully reconstructed. This means that Eq.~\eqref{eq:imagetovideo} simplifies to a mapping onto this representation
\begin{equation}
\mathcal{T}: x_0 \mapsto z_\nu.
\label{eq:imagetovideo2}
\end{equation}
Since $z_\nu$ provides all necessary information to fully reconstruct a video from it, Eq.~\eqref{eq:imagetovideo2} is still highly underspecified, as multiple predictions originate from a given start point $x_0$. This demands a probabilistic model from which possible realizations can be drawn
\begin{equation}
z_\nu \sim p(z_\nu|x_0).
\end{equation}
To implement the mapping in Eq.~\eqref{eq:imagetovideo2}, we thus have to introduce a dedicated \emph{dynamics representation} $\hat{z}_\nu$, such that $\hat{z}_\nu$ and $x_0$ \emph{together} determine a unique mapping from $x_0$ to $z_\nu$, i.e.\
\begin{equation}
z_\nu = \mathcal{T}(\hat{z}_\nu \vert x_0)
\label{eq:forward}
\end{equation}
The problem then reduces to finding the distribution of $\hat{z}_\nu$. 


\paragraph{Inferring An Explicit Dynamic Representation}
To determine $\hat{z}_\nu$, we recall that it has to capture all the information present in the full video representation $z_{\nu}$ \emph{without} the given starting frame $x_0$. This means that $\hat{z}_\nu$ can be determined as the inverse of Eq.~\eqref{eq:forward}
\begin{equation}
\hat{z}_\nu = \mathcal{T}^{-1}(z_\nu \vert x_0), 
\label{eq:backward}
\end{equation}
which exists because the mapping defined by Eq.~\eqref{eq:forward} is assumed to be unique for given $\hat{z}_\nu$ and $x_0$. By the change-of-variables theorem for probability distributions, $\mathcal{T}^{-1}$ transforms $p(z_\nu|x_0)$ as 
\begin{align}
p( z_\nu \vert x_0) &= \frac{p(\hat{z}_\nu \vert x_0)}{\vert \det J_{\mathcal{T}}(\hat{z}_\nu \vert x_0) \vert} \\
&= p(\mathcal{T}^{-1}(z_\nu \vert x_0)) \cdot \vert \det J_{\mathcal{T}^{-1}}(z_\nu \vert x_0) \vert
\label{eq:transformation}
\end{align}
where $J_{\mathcal{T}}$ denotes the Jacobian of the transformation $\mathcal{T}$ and $\vert \det [\cdot] \vert $ the absolute value of the determinant of its input. 

To learn the transformation $\mathcal{T}$, we have to chose a prior $q(\hat{z}_\nu \vert x_0)$ which can be evaluated efficiently and analytically. Furthermore, to assure that $\hat{z}_\nu$ captures only the dynamics and nothing else, we have to make sure that it is independent of the starting frame $x_0$, i.e.\ $q(\hat{z}_\nu \vert x_0) = q(\hat{z}_\nu)$. A straightforward choice for a prior which fulfills these requirements is a standard normal distribution, $q(\hat{z}_\nu) = \mathcal{N}(\hat{z}_\nu \vert 0, \mathbf{1})$. This allows us to implement $\mathcal{T}$ as a conditional invertible neural network, such that Eq.\eqref{eq:transformation} serves as the objective for training $\mathcal{T}$ and the negative log-likelihood can be minimized as 
\begin{align}
\mathcal{L}(\mathcal{T}) &= \mathbb{E}_{z_\nu, x_0} \left[\log q(\mathcal{T}^{-1}(z_\nu \vert x_0)) - \log \vert \det J_{\mathcal{T}^{-1}}(z_\nu \vert x_0) \vert \right] \\
&= \mathbb{E}_{z_\nu, x_0} \left[ \Vert \mathcal{T}^{-1}(z_\nu \vert x_0) \Vert_2^2 -  \log \vert \det J_{\mathcal{T}^{-1}}(z_\nu \vert x_0) \vert + const. \right] .
\end{align}
Note that this is equivalent to minimizing the KL-divergence $\text{KL}[p(\hat{z}_\nu \vert x_0) \Vert q(\hat{z}_\nu)]$. \\
\newline
After training, animating a given starting frame $x_0$ is then performed by first sampling a dynamics, $\hat{z}_\nu \sim q(\hat{z}_\nu)$, and subsequent synthesis of ${x_0, \dots, x_T} = p_\theta(z_\nu|x_0)$ with $z_\nu = \mathcal{T}(\hat{z}_\nu|x_0)$.






In this paper, a novel generative framework is proposed to synthesize diversified videos from a single scenery image. Formally, given a single image $I_0$, our model learns to generate a video sequences $\mathbf{\hat{S}}=\{I_1,I_2,..., I_T\}$ from two disentangled factors: appearance $\alpha$ and dynamic $\pi$. ...
Our new two-stage training procedure 

We aim at generating diverse video sequences $\mathbf{\hat{S}}=\{I_1,I_2,..., I_T\}$ from a starting frame $I_0$. Therefore, we learn a generative model which decomposes dynamics and all other remaining factors e.g. appearance by using a cINN. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% Motivation for two-stage training %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Two-Stage Training Procedure}
\label{Intro_Dis}
We want to learn a generative model that synthesizes diverse sequences by understanding the video sequence $\mathbf{S}$ in terms of two independent factors: appearance, $\alpha$, and dynamics, $\nu$. Ideally, we would like to have access to both independently for sampling new dynamics. The appearance $\alpha$ is naturally independent from dynamic since it can be obtained from a single image $x$. However, the dynamics information $\nu$ is highly entangled in videos with the appearance. Previous work shortcut the problem by using optical flow \cite{Animating_landscapes, dtvnet} or difference images \cite{villegas2018decomposing} to obtain a dynamic representation which is naturally independent from appearance. However, these methods fail when animating textures which cannot be described by apparent pixel displacements, such as fire \cite{two-stream}. In contrast, we approach this difficult task by disentangling appearance from dynamics in a novel way and encode the video sequence $\mathbf{S}$ directly without preprocessing or using optical flow priors.
% The appearance $\alpha$ of a video $\mathbf{S}$ can be obtained from the starting frame $x_0$ and hence is per default independent from motion.
% Consequently, we have to enforce independence between $\alpha$ and $\nu$ and this can be achieved by minimizing the mutual information
\\
Enforcing independence between given factors of variation formally translates to minimizing the mutual information
\begin{align}
I(\alpha, \nu) = D_{\text{KL}}(p(\alpha, \nu)||p(\alpha)p(\nu)).
\label{mutual}
\end{align}
However, directly minimizing this objective is complex since computing reliable estimates of the mutual information is difficult \cite{esser2019unsupervised, belghazi2018mutual}. Previous work \cite{burgess2018understanding, esser2019unsupervised} minimize an upper bound on the mutual information \cite{alex2016deep}
    \begin{align}
    I(\alpha, \nu) \leq D_{\text{KL}}(q_{\phi}(\nu| \mathbf{S}) \| p(\nu)).
\label{eq:upperbound}
\end{align}
by using Variational Autoencoders (VAEs) \cite{VAE, rezende2014stochastic} introducing a variational posterior $q_\phi$. These models are trained to approximate the true data distribution $p(\mathbf{S})$ by optimizing an empirical lower bound (ELBO)
\begin{equation}
\begin{split}
L(p_\theta,q_\phi) := & \; \mathbb{E}_{q_\phi(\nu|\mathbf{S})} \left[ \log p_\theta(\mathbf{S}| \alpha, \nu) \right] \\
& - D_{\text{KL}}(q_\phi(\nu|\mathbf{S})||p(\nu))
\end{split}
\label{eq:elbo}
\end{equation}
with deep neural networks parametrizing $p_\theta$ (the generator) and $q_\phi$ (the encoder), and $p(\nu)$ being the prior on the posterior $q_\phi$. The first term optimizes the synthesis quality of the generator while the second regularizes the encoder to match the prior and, as a result, minimizes also the upper bound in Eq.~\ref{eq:upperbound}.
%% 2 problems:
% (i) log likelihood stands in in contrast to regularization term -> trade off between disentanglement and synthesis quality
% (ii) log likelihood depends on the expressiveness of z_D. minimizing mutual information leads to information reduction of z_D
However, the trade-off between synthesis and regularization in optimizing Eq.~\ref{eq:elbo} leads to a reduction of generation quality \cite{chen2016variational, zhao2017infovae}. This becomes evident as the log-likelihood depends on the expressiveness of $\nu$ which is decreased by Eq.~\ref{eq:upperbound}. Moreover, the sampling diversity also depends on the expressiveness of $\nu$, and thus is also diminished. 
\\
% \red{To alleviate this problem, we propose to optimize both terms in Eq.~\ref{eq:elbo} separately which leads to a two stage training approach. In the first stage, we optimize the log likelihood to achieve optimal synthesis quality. Consequently, this leads to an intermediate latent representation $\nu$ which will not be disentangled from appearance. Therefore, we subtract the appearance in the second stage by introducing a bijective transformation to an additional representation $\hat{\nu}$ in which we enforce independence by minimizing Eq~\ref{eq:upperbound}. Through the bijective transformation we are able to sample new dynamics and by that synthesize novel videos.}.
To alleviate this problem, we propose to optimize each term of Eq.~\ref{eq:elbo} individually in separate, consecutive training stages: The first stage directly optimizes the log-likelidhood. While this leads to optimal synthesis quality, the resulting latent representation $\nu$ will in general not be disentangled from appearance. This shortcoming is subsequently addressed in a second training stage which is formulated to discard the remaining appearance information from the (intermediate) latent representation $\nu$. To this end, we learn a conditional bijective transformation of $\nu$ to a dedicated dynamics space $\hat{\nu}$ while enforcing minimal mutual information with $\alpha$ (cf. Eq.~\ref{eq:upperbound}). The synthesis of novel dynamics and, thus, videos proceeds by first sampling dynamics from $\hat{\nu}$, then translating it to $\nu$ conditioned on a target appearance $\alpha$, and finally decoding to the video domain using the generator.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% STAGE 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Synthesis of video sequences animating a starting image $x_0$ depicting the appearance $\alpha$ with diverse, plausible dynamics $\nu$ requires to carefully model the interplay between both factors. To this end, we propose a NOVEL video residual module designed to optimally combine motion and appearance at each scale of the generation process. 
\subsection{Video-to-Video Stage}
In the first stage, we introduce a new video residual block for the generator, $p_{\theta}$, which combines appearance, $\alpha$, and dynamics, $\nu$, to maximize the log-likelihood. 
The generator consists of $n$ video residual block in which the dynamic as well as the appearance information are combined at all scales and by that, allowing a natural information flow throughout the generator. In Figure \ref{fig:method1}, of the generator as well as the structure of the residual block is illustrated. 
\\
The first module in the video residual block is a SPADE \cite{spade} normalization layer to preserve semantics throughout the generator. For that, the conditioning image $x_0$ is down-sampled to the corresponding feature map size. The statistics of the normalization layer are learned with convolutions from $x_0$. 
% by which the activations $\mathbf{h}^i$ of the i-th layer are transformed according to 
    % \begin{align}
    %     \gamma^i_{c, y, x} (x_0) \frac{h^i_{n, t, c, y, x} -  \mu^i}{\sigma^i}  + \beta^i_{c, y, x} (\alpha)
    % \end{align}
    % with $C^i$ the number of channels, $T^i$ the temporal length and $H^i, W^i$ the height and width of the activation map. The variables $\gamma^i_{c, y, x} (x_0)$ and $\beta^i_{c, y, x} (x_0)$ are the learned modulation parameters. 
After applying an activation function as well as a 3D convolution, the dynamics information is incorporated through an ADAIN \cite{karras2019stylebased} layer.
% by which the activations $\mathbf{h}^i$ of the i-th layer are transformed according to
% \begin{align}
%     \gamma^i_{c} (\nu) \frac{h^i_{n, t, c, y, x} -  \mu^i}{\sigma^i}  + \beta^i_{c} (\nu) .
% \end{align}
Note, the learned variables for the normalization do not have spatial expansions. This is crucial since the network would otherwise learn a shortcut by representing an optical flow like structure. Informally, by removing the spatial dimensions we are treating the dynamics as the 'style' of the video.
\\
We model the true data distribution as a parametric Laplace with constant standard deviation and assume that $p_{\theta}$ is deterministic in $\mathbf{S}$, following common practice \cite{VAE}. Thus $p_{\theta}$ can be considered to be an video generator and the log likelihood can be rewritten as a $L_1$ objective. Since the $L_1$ norm does not model perceptual quality \cite{larsen2016autoencoding} we add the perceptual loss $\ell^{\phi}$ \cite{dosovitskiy201perceptual, johnson2016perceptual} to our objective. 
To further improve the synthesis quality we follow previous work \cite{DVDGAN, vid2vid} by using one discriminator on the frame level $\mathcal{D}_S$ and one $\mathcal{D}_T$ on the temporal level. The hinge formulation \cite{lim2017geometric, big_gan_brock} is used as the objective for the GAN training. The objective for our generator $p_{\theta}$ can be summarized as follows:
\begin{equation}
\begin{split}
    \mathcal{L} &= \frac{\lambda_1}{T} [ \sum_{i=1}^{T}\parallel x_i - p_\theta(\alpha, \nu)_i \parallel_1 +  \sum_{i=1}^{T}\ell^{\phi}(x_i, p_\theta(\alpha, \nu)_i) ] \\
    &- \lambda_2 \mathcal{D}_T(p_\theta(\alpha, \nu)) - \lambda_3 \mathcal{D}_S(p_\theta(\alpha, \nu)) 
\end{split}
\end{equation}

%-torch.mean(pred_gen)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% STAGE 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Image-to-Video Stage}
% Since the first stage exclusively optimizes our generator to synthesize visually appealing video sequences, the intermediate dynamics representation, $\nu$, is in general not disentangled from $\alpha$. To compensate for this shortcoming, we now learn a transformation, $\mathcal{T}$, to discount the remaining appearance information, thus yielding a dedicated dynamics representation $\hat{\nu}$. Moreover, for manipulating the dynamics captured by $\hat{\nu}$ to affect the synthesis process, $p_\theta(\mathbf{S}| \alpha, \nu)$, $\mathcal{T}$ is required to be invertible, i.e., it allows to return to the original representation $\nu$ by combining the appearance $\alpha$ and dynamics $\hat{\nu}$. 

Write down as domain transfer image-to-video synthesis. 
While such invertible transformations have been applied to inverse problems \cite{ardizzone2019analyzing}, domain transfer \cite{esser2020disentangling, rombach2020making, rombach2020network}, unconditional image synthesis \cite{kingma2018glow, pumarola2020cflow} and representation learning \cite{jacobsen2018irevnet}, we use $\mathcal{T}$ to effectively disentangle appearance and dynamics without interfering with the first stage model.
\\
Formally, we seek a conditional bijective mapping $\mathcal{T}(\nu|\alpha)$ between $\nu$ and $\hat{\nu}$, such that $\hat{\nu}$ represents the dynamics distribution independent of appearance, $\alpha$. Considering the lower bound on the mutual information in Eq. \ref{eq:upperbound}, i.e.,
\begin{align}
    I(\alpha, \hat{\nu}) &\leq D_{KL}(p(\hat{\nu}|\alpha) \| q(\hat{\nu})) \\
    &= \int_{\hat{\nu}} p(\hat{\nu}|\alpha) \log \frac{p(\hat{\nu}|\alpha)}{q(\hat{\nu})} \; ,
    % &= \int_{\nu} p(\mathcal{T}(\nu|\alpha)|\alpha) \log \frac{p(\mathcal{T}(\nu|\alpha)|\alpha)}{q(\mathcal{T}(\nu|\alpha))} |\det _\mathcal{T}(\nu|\alpha)|
\end{align}
and inserting $\mathcal{T}(\nu|\alpha)$ we arrive at
\begin{equation}
\begin{aligned}
    I(\alpha, \hat{\nu}) \leq \mathbb{E}_{\nu} \{&- \log q(\mathcal{T}(\nu|\alpha)) + \log p(\nu|\alpha)\\
    &- \log |\det J_{\mathcal{T}}(\nu|\alpha)|  \}
\end{aligned}
\label{eq:cINN}
\end{equation}
using the inverse function theorem (for more details, see supplementary material). By neglecting the constant term $\log p(\nu|\alpha)$, we thus obtain a transformed upper bound on the mutual information to enforce the desired disentanglement. The procedure is visualized in Figure~\ref{fig:method2} left. This transformation is implemented with a conditional Invertible Neural Network (cINN) which learns a bijective transformation $\mathcal{T} = h_{\xi_1} \circ h_{\xi_2} \circ \dots \circ h_{\xi_D}$ with $D$ invertible functions, $h_{\xi_j}$, parametrized by $\xi_j$ to a prior distribution $\hat{\nu} \sim q(\hat{\nu})$. The prior distribution is realized as a standard Gaussian.
\\
An informal explanation of the disentanglement process is given by the universality property of autoregressive flows \cite{Kobyzev_INN_survey_2020}: INNs can learn any target distribution $q_\phi(\nu$) to any required precision given sufficient data and capacity. However, both the capacity and and training data is limited during training. Thus, maximal precision can only be achieved by extracting appearance, $\alpha$, directly from the readily available conditioning image $x_0$ and dedicating as much capacity as possible for capturing the residual information, i.e., the dynamics, in $q(\hat{\nu})$. 
%conditioning the transformation on an additional factors e.g. appearance $\alpha$ forces the INN to spare computation. Hence, independence is achieved since the INN does not require to represent any of the conditioning in the target representation.
\\
Animating a given starting frame $x_0$ with appearance, $\alpha$, is then performed by first sampling a dynamics, $\hat{\nu}^* \sim q(\hat{\nu})$, and subsequent synthesis of $\mathbf{S} = p_\theta(\nu|\alpha)$ with $\nu = \mathcal{T}^{-1}(\hat{\nu}|\alpha)$.
